Sum-Product Network Decompilation

There exists a dichotomy between classical probabilistic graphical models, such as Bayesian networks (BNs), and modern tractable models, such as sum-product networks (SPNs). The former generally have intractable inference, but provide a high level of interpretability, while the latter admits a wide range of tractable inference routines, but are typically harder to interpret. Due to this dichotomy, tools to convert between BNs and SPNs are desirable. While one direction -- compiling BNs into SPNs -- is well discussed in Darwiche's seminal work on arithmetic circuit compilation, the converse direction -- decompiling SPNs into BNs -- has received surprisingly little attention. In this paper, we fill this gap by proposing SPN2BN, an algorithm that decompiles an SPN into a BN. SPN2BN has several salient features when compared to the only other two works decompiling SPNs. Most significantly, the BNs returned by SPN2BN are minimal independence-maps that are more parsimonious with respect to the introduction of latent variables. Secondly, the output BN produced by SPN2BN can be precisely characterized with respect to a compiled BN. More specifically, a certain set of directed edges will be added to the input BN, giving what we will call the moral-closure. Lastly, it is established that our compilation-decompilation process is idempotent. This has practical significance as it limits the size of the decompiled SPN.

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}

% GRANT: 238880
This research is partially supported by NSERC Discovery Grant XXXXXX and has also received funding from the European Union's Horizon 2020 research and innovation programme under the Marie Sk\l{}odowska-Curie Grant Agreement No.~797223 --- HYBSPN.

==> sections/experiments.tex <==
\section{Synthetic Experiments}
\label{sec:exp}

In this section, we first reaffirm our result in Theorem \ref{th:rec_moral} with systematic experiments on a number of synthetic BNs.
Next, we show how our decompilation method SPN2BN can enhance interpretability of an SPN learned from data.

\subsection{Empirical Analysis on the Moral Closure}

We empirically tested Theorem \ref{th:rec_moral} by verifying whether the output BN of BN2SPN2BN was the moral closure ${\cal B}^c$ of the input BN ${\cal B}$.

For a fixed number $N$ of variables  $X_1, \ldots, X_N$, we exhaustively construct all possible connected BNs that are consistent with ordering $1,\ldots,N$.
Using different orderings would amount to relabelings of the variables in our synthetic BNs and return the corresponding relabeled SPN and BN structures.

Table \ref{tab:set2} describes our experiments.
The number of variables $N$ ran from 2 through 7 inclusive.
The number of possible BNs is given in the second line.
The total number of possible elimination orderings is given in the third line.
Finally, the last row reports the total number of trials that were conducted, which is simply the product of the first two rows.
In each and every case, our compilation-decompilation process returned the moral closure ${\cal B}^c$ of the input BN ${\cal B}$.
This empirically confirms our theoretical findings.

\begin{table}[tb]
    \caption{Synthetic BN characteristics.}
    \label{tab:set2}
    \begin{tabular}{l|llllllllllllllllllllll}
    \# vars       & 2 & 3 & 4 & 5 & 6 & 7 \\
    \hline
    \# BNs    &   1  &   3  &   21  &   315  &  9.8K   &  615K   \\
    \# elim ord &   1  &   2  &  6   &   24  &   120  &  720   \\
    \# trials &   1  &   6  &  126   &   7.6K  &   1.2M  & 443M
    \end{tabular}
\end{table}

\subsection{SPN Decompilation and Interpretability}

We want to demonstrate how the decompilation algorithm can be used to better understand an SPN learned from data.
% Let us we decompile the well-known SPN structure, called a region graph, first suggested in \cite{poon2011sum}.

% The SPN structure in \cite{poon2011sum} leverages local structure in an image dataset.
% The idea is to select all rectangular regions, with the smallest regions corresponding to pixels.
% Subsequently, for each rectangular region, all possible ways to decompose it into two rectangular subregions are considered.
% This recursive procedure yields a valid SPN structure formed by layers of sum and product nodes, known as a \emph{region graph} \cite{dennis2012learning,peharz2018probabilistic}.
% By construction, given the height and width of an image, a region graph is unique.

% We ran experiments decompiling some fixed-size region graphs.
% Consider an image of size 3-by-3.
% The region graph for such an image is depicted in Figure \ref{fig:pnd} (\subref{subfig:spn_pnd}).
% We used SPN2BN to decompile the region graph into the BN in Figure \ref{fig:pnd} (\subref{subfig:bn_pnd}).

% \begin{figure*}[tb]
%     \begin{center}
%     \begin{subfigure}[t]{0.40\linewidth}
%       \centering
%         \includegraphics[width=\linewidth]{figures/spn_pnd.png}
%            \caption{}
%            \label{subfig:spn_pnd}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.40\linewidth}
%       \centering
%         \includegraphics[width=\linewidth]{figures/bn_pnd.png}
%            \caption{}
%            \label{subfig:bn_pnd}
%     \end{subfigure}
%     \caption{An SPN structure (a region graph) for a 3-by-3 image in (\subref{subfig:spn_pnd}). In (\subref{subfig:bn_pnd}), the decompiled BN using Algorithm \ref{alg:decomp}.}
%     \label{fig:pnd}
%     \end{center}
%   \end{figure*}

We can read independence information for the decompiled SPN using d-separation.
% For instance, observing variables in the second layer (from bottom to top) of ${\cal B}$ renders some variables of the third layer dependent on each other.
These independencies can help the interpretability of SPN applications, including autoencoders.
In \cite{Vergari2018qu}, visualization of the latent space shows that the deeper the SPN layer, the higher the level of complexity being learned.
They consider the \emph{mnist} dataset of handwriting digits.
Visualizing the input layer of an SPN learned on mnist shows primitive drawings such as circular and linear forms, while hidden layers show segments of digits.
Thus, a decompiled BN for this SPN encodes independencies and dependencies between the circular/linear forms and the segments of digits.

